An Approach for Addressing Internally-Disconnected Communities in Louvain Algorithm

Community detection is the problem of identifying densely connected clusters within a network. While the Louvain algorithm is commonly used for this task, it can produce internally-disconnected communities. To address this, the Leiden algorithm was introduced. This technical report introduces GSP-Louvain, a parallel algorithm based on Louvain, which mitigates this issue. Running on a system with two 16-core Intel Xeon Gold 6226R processors, GSP-Louvain outperforms Leiden, NetworKit Leiden, and cuGraph Leiden by 391x, 6.9x, and 2.6x respectively, processing 410M edges per second on a 3.8B edge graph. Furthermore, GSP-Louvain improves performance at a rate of 1.5x for every doubling of threads.

==> src/alg-leiden.tex <==
\begin{algorithm}[hbtp]
\caption{GSP-Leiden: Our Parallel Leiden algorithm which returns communities that are not internally disconnected.}
\label{alg:leiden}
\begin{algorithmic}[1]
\Require{$G(V, E)$: Input graph}
\Ensure{$G'(V', E')$: Input/super-vertex graph}
\Ensure{$C$: Community membership of each vertex}
\Ensure{$C'$: Community membership of each vertex in $G'$}
\Ensure{$K'$: Total edge weight of each vertex}
\Ensure{$\Sigma'$: Total edge weight of each community}
\Ensure{$l_i$, $l_j$: Number of iterations performed (per pass)}
\Ensure{$l_p$: Number of passes performed}
\Ensure{$\tau, \tau_{agg}$: Iteration, Aggregation tolerance}

\Statex

\Function{leiden}{$G$} \label{alg:leiden--begin}
  \State Vertex membership: $C \gets [0 .. |V|)$ \textbf{;} $G' \gets G$ \label{alg:leiden--initialization}
  \ForAll{$l_p \in [0 .. \text{\small{MAX\_PASSES}})$} \label{alg:leiden--passes-begin}
    \State $\Sigma' \gets K' \gets vertexWeights(G')$ \textbf{;} $C' \gets [0 .. |V'|)$ \label{alg:leiden--reset-weights}
    \State $l_i \gets commonMove(G', C', K', \Sigma', \tau)$ \Comment{Algorithm \ref{alg:commonlm}} \label{alg:leiden--local-move}
    \State $C'_B \gets C'$ \textbf{;} $C' \gets [0 .. |V'|)$ \textbf{;} $\Sigma' \gets K'$ \label{alg:leiden--reset-again}
    \State $l_j \gets leidenRefine(G', C'_B, C', K', \Sigma', \tau)$ \Comment{Algorithm \ref{alg:leidenre}} \label{alg:leiden--refine}
    \State $C' \gets splitDisconnectedBfs(G', C')$ \Comment{Algorithm \ref{alg:splitbfs}} \label{alg:leiden--split}
    \If{$l_i + l_j \le 1$} \textbf{break} \Comment{Globally converged?} \label{alg:leiden--globally-converged}
    \EndIf
    \State $|\Gamma|, |\Gamma_{old}| \gets$ Number of communities in $C$, $C'$
    \If{$|\Gamma|/|\Gamma_{old}| > \tau_{agg}$} \textbf{break} \Comment{Low shrink?} \label{alg:leiden--aggregation-tolerance}
    \EndIf
    \State $C' \gets$ Renumber communities in $C'$ \label{alg:leiden--renumber}
    \State $C \gets$ Lookup dendrogram using $C$ to $C'$ \label{alg:leiden--lookup}
    \State $G' \gets commonAggregate(G', C')$ \Comment{Algorithm \ref{alg:commonag}} \label{alg:leiden--aggregate}
    \State $\tau \gets \tau / \text{\small{TOLERANCE\_DROP}}$ \Comment{Threshold scaling} \label{alg:leiden--threshold-scaling}
  \EndFor \label{alg:leiden--passes-end}
  \State $C \gets$ Lookup dendrogram using $C$ to $C'$ \label{alg:leiden--lookup-last}
  \Return{$C$} \label{alg:leiden--return}
\EndFunction \label{alg:leiden--end}
\end{algorithmic}
\end{algorithm}


==> src/alg-leidenag.tex <==
\begin{algorithm}[hbtp]
\caption{Aggregation phase of GSP-Leiden \cite{sahu2023gveleiden}.}
\label{alg:leidenag}
\begin{algorithmic}[1]
\Require{$G'(V', E')$: Input/super-vertex graph}
\Require{$C'$: Community membership of each vertex}
\Ensure{$G'_{C'}(V'_{C'}, E'_{C'})$: Community vertices (CSR)}
\Ensure{$G''(V'', E'')$: Super-vertex graph (weighted CSR)}
\Ensure{$*.offsets$: Offsets array of a CSR graph}
\Ensure{$H_t$: Collision-free per-thread hashtable}

\Statex

\Function{leidenAggregate}{$G', C'$}
  \State $\rhd$ Obtain vertices belonging to each community
  \State $G'_{C'}.offsets \gets countCommunityVertices(G', C')$ \label{alg:leidenag--coff-begin}
  \State $G'_{C'}.offsets \gets exclusiveScan(G'_{C'}.offsets)$ \label{alg:leidenag--coff-end}
  \ForAll{$i \in V'$ \textbf{in parallel}} \label{alg:leidenag--comv-begin}
    \State Add edge $(C'[i], i)$ to CSR $G'_{C'}$ atomically
  \EndFor \label{alg:leidenag--comv-end}
  \State $\rhd$ Obtain super-vertex graph
  \State $G''.offsets \gets communityTotalDegree(G', C')$ \label{alg:leidenag--yoff-begin}
  \State $G''.offsets \gets exclusiveScan(G''.offsets)$ \label{alg:leidenag--yoff-end}
  \State $|\Gamma| \gets$ Number of communities in $C'$
  \ForAll{$c \in [0, |\Gamma|)$ \textbf{in parallel}} \label{alg:leidenag--y-begin}
    \If{degree of $c$ in $G'_{C'} = 0$} \textbf{continue}
    \EndIf
    \State $H_t \gets \{\}$
    \ForAll{$i \in G'_{C'}.edges(c)$}
      \State $H_t \gets scanCommunities(H, G', C', i, true)$
    \EndFor
    \ForAll{$(d, w) \in H_t$}
      \State Add edge $(c, d, w)$ to CSR $G''$ atomically
    \EndFor
  \EndFor \label{alg:leidenag--y-end}
  \Return $G''$ \label{alg:leidenag--return}
\EndFunction
\end{algorithmic}
\end{algorithm}


==> src/alg-leidenlm.tex <==
\begin{algorithm}[hbtp]
\caption{Local-moving phase of GVE-Leiden.}
\label{alg:leidenlm}
\begin{algorithmic}[1]
\Require{$G'(V', E')$: Input/super-vertex graph}
\Require{$C'$: Community membership of each vertex}
\Require{$K'$: Total edge weight of each vertex}
\Require{$\Sigma'$: Total edge weight of each community}
\Ensure{$G'_{C'}$: Community vertices (CSR)}
\Ensure{$H_t$: Collision-free per-thread hashtable}
\Ensure{$l_i$: Number of iterations performed}
\Ensure{$\tau$: Per iteration tolerance}

\Statex

\Function{leidenMove}{$G', C', K', \Sigma', \tau$} \label{alg:leidenlm--move-begin}
  \State Mark all vertices in $G'$ as unprocessed \label{alg:leidenlm--reset-affected}
  \ForAll{$l_i \in [0 .. \text{\small{MAX\_ITERATIONS}})$} \label{alg:leidenlm--iterations-begin}
    \State Total delta-modularity per iteration: $\Delta Q \gets 0$ \label{alg:leidenlm--init-deltaq}
    \ForAll{unprocessed $i \in V'$ \textbf{in parallel}} \label{alg:leidenlm--loop-vertices-begin}
      \State Mark $i$ as processed (prune) \label{alg:leidenlm--prune}
      \State $H_t \gets scanCommunities(\{\}, G', C', i, false)$ \label{alg:leidenlm--scan}
      \State $\rhd$ Use $H_t, K', \Sigma'$ to choose best community
      \State $c^* \gets$ Best community linked to $i$ in $G'$ \label{alg:leidenlm--best-community-begin}
      \State $\delta Q^* \gets$ Delta-modularity of moving $i$ to $c^*$ \label{alg:leidenlm--best-community-end}
      \If{$c^* = C'[i]$} \textbf{continue} \label{alg:leidenlm--best-community-same}
      \EndIf
      \State $\Sigma'[C'[i]] -= K'[i]$ \textbf{;} $\Sigma'[c^*] += K'[i]$ \textbf{atomic} \label{alg:leidenlm--perform-move-begin}
      \State $C'[i] \gets c^*$ \textbf{;} $\Delta Q \gets \Delta Q + \delta Q^*$ \label{alg:leidenlm--perform-move-end}
      \State Mark neighbors of $i$ as unprocessed \label{alg:leidenlm--remark}
    \EndFor \label{alg:leidenlm--loop-vertices-end}
    \If{$\Delta Q \le \tau$} \textbf{break} \Comment{Locally converged?} \label{alg:leidenlm--locally-converged}
    \EndIf
  \EndFor \label{alg:leidenlm--iterations-end}
  \Return{$l_i$} \label{alg:leidenlm--return}
\EndFunction \label{alg:leidenlm--move-end}

\Statex

\Function{scanCommunities}{$H_t, G', C', i, self$}
  \ForAll{$(j, w) \in G'.edges(i)$}
    \If{\textbf{not} $self$ \textbf{and} $i = j$} \textbf{continue}
    \EndIf
    \State $H_t[C'[j]] \gets H_t[C'[j]] + w$
  \EndFor
  \Return{$H_t$}
\EndFunction
\end{algorithmic}
\end{algorithm}


==> src/alg-leidenre.tex <==
\begin{algorithm}[hbtp]
\caption{Refinement phase of GSP-Leiden.}
\label{alg:leidenre}
\begin{algorithmic}[1]
\Require{$G'(V', E')$: Input/super-vertex graph}
\Require{$C'_B$: Community bound of each vertex}
\Require{$C'$: Community membership of each vertex}
\Require{$K'$: Total edge weight of each vertex}
\Require{$\Sigma'$: Total edge weight of each community}
\Require{$\tau$: Iteration tolerance}
\Ensure{$H_t$: Collision-free per-thread hashtable}
\Ensure{$l_j$: Number of iterations performed}

\Statex

\Function{leidenRefine}{$G', C'_B, C', K', \Sigma', \tau$} \label{alg:leidenre--move-begin}
  \State Mark all vertices in $G'$ as unprocessed \label{alg:leidenre--reset-affected}
  \ForAll{$l_j \in [0 .. \text{\small{MAX\_ITERATIONS}})$} \label{alg:leidenre--iterations-begin}
    \State Total delta-modularity per iteration: $\Delta Q \gets 0$ \label{alg:leidenre--init-deltaq}
    \ForAll{unprocessed $i \in V'$ \textbf{in parallel}} \label{alg:leidenre--loop-vertices-begin}
      \State Mark $i$ as processed (prune) \label{alg:leidenre--prune}
      \State $H_t \gets scanBounded(\{\}, G', C'_B, C', i, false)$ \label{alg:leidenre--scan}
      \State $\rhd$ Use $H_t, K', \Sigma'$ to choose best community
      \State $c^* \gets$ Best community linked to $i$ in $G'$ within $C'_B$ \label{alg:leidenre--best-community-begin}
      \State $\delta Q^* \gets$ Delta-modularity of moving $i$ to $c^*$ \label{alg:leidenre--best-community-end}
      \If{$c^* = C'[i]$} \textbf{continue} \label{alg:leidenre--best-community-same}
      \EndIf
      \State $\Sigma'[C'[i]] -= K'[i]$ \textbf{;} $\Sigma'[c^*] += K'[i]$ \textbf{atomic} \label{alg:leidenre--perform-move-begin}
      \State $C'[i] \gets c^*$ \textbf{;} $\Delta Q \gets \Delta Q + \delta Q^*$ \label{alg:leidenre--perform-move-end}
      \State Mark neighbors of $i$ as unprocessed \label{alg:leidenre--remark}
    \EndFor \label{alg:leidenre--loop-vertices-end}
    \If{$\Delta Q \le \tau$} \textbf{break} \Comment{Locally converged?} \label{alg:leidenre--locally-converged}
    \EndIf
  \EndFor \label{alg:leidenre--iterations-end}
  \Return{$l_j$} \label{alg:leidenre--return}
\EndFunction \label{alg:leidenre--move-end}

\Statex

\Function{scanBounded}{$H_t, G', C'_B, C', i, self$}
  \ForAll{$(j, w) \in G'.edges(i)$}
    \If{\textbf{not} $self$ \textbf{and} $i = j$} \textbf{continue}
    \EndIf
    \If{$C'_B[i] \neq C'_B[j]$} \textbf{continue}
    \EndIf
    \State $H_t[C'[j]] \gets H_t[C'[j]] + w$
  \EndFor
  \Return{$H_t$}
\EndFunction
\end{algorithmic}
\end{algorithm}


==> src/fig-onleiden.tex <==
\begin{figure*}[hbtp]
  \centering
  \subfigure[Community $C1$ is internally disconnected]{
    \label{fig:onleiden--1}
    \includegraphics[width=0.31\linewidth]{out/onleiden-1.pdf}
  }
  \subfigure[Upon refinement $C1$ splits into $C3$, $C4$, and $C5$]{
    \label{fig:onleiden--2}
    \includegraphics[width=0.31\linewidth]{out/onleiden-2.pdf}
  }
  \subfigure[With further refinement, vertex $5$ joins $C4$]{
    \label{fig:onleiden--3}
    \includegraphics[width=0.31\linewidth]{out/onleiden-3.pdf}
  }
  \subfigure[Upon aggregation, if the community assignment for refined partitions is based on the local-moving phase, the community $C1$ is still disconnected]{
    \label{fig:onleiden--4}
    \includegraphics[width=0.31\linewidth]{out/onleiden-4.pdf}
  }
  \hspace{8ex}
  \subfigure[Upon aggregation, if the community assignment for refined partitions is based on the refinement phase, the community $C3$ remains disconnected]{
    \label{fig:onleiden--5}
    \includegraphics[width=0.31\linewidth]{out/onleiden-5.pdf}
  } \\[-2ex]
  \caption{An example demonstrating the possibility of internally disconnected communities with the Leiden algorithm. Here, $C1$ and $C2$ are two communities obtained after running some iterations of the Louvain algorithm, where the community $C1$ is internally disconnected --- similar to the scenario in Figure \ref{fig:onlouvain--3}. Vertices $1$ to $6$ and vertices $8$ to $10$ are members of community $C1$, while the vertex $7$ has joined the community $C2$, after having acted as a bridge for $C1$. Upon performing the refinement phase, the community $C1$ splits into communities $C3$, $C4$, and $C5$ after a few iterations (starting from singleton partitions). In a subsequent iteration, suppose vertex $5$ leaves $C3$, and joins $C4$ instead. This causes the $C3$ to be internally disconnected. Finally, (d) and (e) present how disconnected communities continue to persist, depending upon how the community assignments for super-vertices are made (with (d) being the recommended approach by Traag et al. \cite{com-traag19}). In the figure, ellipses are used to indicate super-vertices in the aggregated graph, and thick lines are used to denote higher edge weights.}
  \label{fig:onleiden}
\end{figure*}


==> src/fig-optduo.tex <==
\begin{figure}[hbtp]
  \centering
  \subfigure[Relative runtime for Parallel Louvain algorithm, and \textit{light}, \textit{medium}, and \textit{heavy} variants of Parallel Leiden algorithm]{
    \label{fig:optduo--runtime}
    \includegraphics[width=0.98\linewidth]{out/optduo-runtime.pdf}
  } \\[-0ex]
  \subfigure[Modularity of communities obtained for Parallel Louvain algorithm, and \textit{light}, \textit{medium}, and \textit{heavy} variants of Parallel Leiden algorithm]{
    \label{fig:optduo--modularity}
    \includegraphics[width=0.98\linewidth]{out/optduo-modularity.pdf}
  } \\[-0ex]
  \subfigure[Fraction of disconnected communities for Parallel Louvain algorithm, and \textit{light}, \textit{medium}, and \textit{heavy} variants of Parallel Leiden algorithm]{
    \label{fig:optduo--disconnected}
    \includegraphics[width=0.98\linewidth]{out/optduo-disconnected.pdf}
  } \\[-2ex]
  \caption{Mean relative runtime, modularity, and fraction of disconnected communities using the \textit{light}, \textit{medium}, and \textit{greedy} variants of Parallel Leiden algorithm \cite{sahu2023gveleiden} across all graphs in the dataset. Additionally, details for Parallel Louvain algorithm \cite{sahu2023gvelouvain} are included as a reference.}
  \label{fig:optduo}
\end{figure}


==> src/fig-optleisp.tex <==
\begin{figure}[hbtp]
  \centering
  \subfigure[Relative runtime using different approaches for splitting disconnected communities with Parallel Leiden algorithm]{
    \label{fig:optleisp--runtime}
    \includegraphics[width=0.98\linewidth]{out/optleisp-runtime.pdf}
  } \\[-0ex]
  \subfigure[Modularity of communities obtained using different approaches for splitting disconnected communities with Parallel Leiden algorithm]{
    \label{fig:optleisp--modularity}
    \includegraphics[width=0.98\linewidth]{out/optleisp-modularity.pdf}
  } \\[-0ex]
  \subfigure[Fraction of disconnected communities (logarithmic scale) using different approaches for splitting disconnected communities with Parallel Leiden algorithm]{
    \label{fig:optleisp--disconnected}
    \includegraphics[width=0.98\linewidth]{out/optleisp-disconnected.pdf}
  } \\[-2ex]
  \caption{Mean relative runtime, modularity, and fraction of disconnected communities (log-scale) using \textit{Split Last (SL)} and \textit{Split Pass (SP)} approaches for splitting disconnected communities with Parallel Leiden algorithm \cite{sahu2023gveleiden} across all graphs in the dataset. Both \textit{SL} and \textit{SP} approaches employ\ignore{minimum label-based} \textit{Label Propagation (LP)}, \textit{Label Propagation with Pruning (LPP)}, or \textit{Breadth First Search (BFS)} techniques for splitting.}
  \label{fig:optleisp}
\end{figure}


==> src/fig-splitleisp.tex <==
\begin{figure*}[hbtp]
  \centering
  \subfigure[Phase split of \textit{GSP-Leiden}]{
    \label{fig:splitleisp--phase}
    \includegraphics[width=0.48\linewidth]{out/splitleisp-phases.pdf}
  }
  \subfigure[Pass split of \textit{GSP-Leiden}]{
    \label{fig:splitleisp--pass}
    \includegraphics[width=0.48\linewidth]{out/splitleisp-passes.pdf}
  } \\[-2ex]
  \caption{Phase split of \textit{GSP-Leiden} shown on the left, and pass split shown on the right for each graph in the dataset.}
  \label{fig:splitleisp}
\end{figure*}

